TIPS: Mining Top-K Locations to Minimize User-Inconvenience for Trajectory-Aware Services

Facility location problems aim to identify the best locations to set up new services. Majority of the existing works typically assume that the users are static. However, there exists a wide array of services such as fuel stations, ATMs, food joints, etc., that are widely accessed by mobile users besides the static ones. Such trajectory-aware services should, therefore, factor in the trajectories of its users rather than simply their static locations. In this work, we introduce the problem of optimal placement of facility locations for such trajectory-aware services that minimize the user inconvenience. The inconvenience of a user is the extra distance traveled by her from her regular path to avail a service. We call this the TIPS problem (Trajectory-aware Inconvenience-minimizing Placement of Services) and consider two variants of it. The goal of the first variant, MAXTIPS, is to minimize the maximum inconvenience faced by any user, while that of the second, AVGTIPS, is to minimize the average inconvenience over all the users. We show that both these problems are NP-hard, and propose multiple efficient heuristics to solve them. Empirical evaluation on real urban-scale road networks validate the efficiency and effectiveness of the proposed heuristics.

==> existing.tex <==
\section{Handling Existing Services}
\label{sec:existing}


Optimal location queries usually factor in existing service locations while
planning for new ones.  We next show how the heuristics presented in
Sec.~\ref{sec:maxtips} and Sec.~\ref{sec:meantips} can be easily adapted to
handle an existing set of services, denoted by $\q_0$. 
\comment{
In each of the proposed algorithms, we initialize the answer set $\q \leftarrow \q_0$.
}
Consider \maxtips problem with input parameters $(k,\ufs)$. 

\noindent
%
\comment{
\textbf{\fftwo:} As an initialization step, for each site in $\q_0$, we pick
the nearest trajectory and add it to the set \reptraj. Then the trajectory
selection phase is performed. Note that at this stage, the trajectories in
\reptraj are placed as far as possible from each other.  Before the site
selection phase begins, we prune the trajectories in \reptraj that were added
in the initialization step. This is because there are already existing services
in their vicinity. The rest of the algorithm stays unchanged. 
}

\begin{itemize}

	\item \textbf{\mif:} The algorithm begins with the following sets
		initialized as follows:$\q \leftarrow \q_0$, and $\reptraj \leftarrow
		\varnothing$. The \nn maps are updated to reflect the nearest facility
		in \q for each trajectory along with its distance.  The algorithm
		begins by choosing the trajectory that is at rank $\trajthres -
		|\reptraj|$ in the sorted ordering of distances in \nn. The rest of the
		algorithm remains unchanged.

	\item \textbf{\nc:} During each binary search call to the \nc framework
		with parameters $(k,\tau)$, the set \q is initialized with $\q_0$.
		Those trajectories that are within the coverage threshold $\tau$ of any
		of the existing facilities are deemed to be served.  The marginal
		utilities of remaining candidate sites are updated by considering this.
		The remaining algorithm remains unaltered.

\end{itemize}

Now consider \meantips problem with input parameter $k$. Each of the algorithms, \hcc and \incg, begins by initializing $\q \leftarrow \q_0$ and updating the \nn maps to
account for the existing services.

\begin{itemize}

	\item \textbf{\incg:} No change is required.

	\item \textbf{\hcc:} After the initialization step, a random set of $k$
		sites in \s is added to \q. The members of \q are referred to as
		medoids. The swaps between medoids and non-medoids do not consider the
		medoids in $\q_0$ as they correspond to the existing service locations.
		The remaining algorithm remains unchanged.

\end{itemize}

\comment{
\noindent
%
$\bullet$ \textbf{\incg:} The rest of the algorithm remains the same.
}

